Generalized Rank Pooling for Activity Recognition

Most popular deep models for action recognition split video sequences into short sub-sequences consisting of a few frames; frame-based features are then pooled for recognizing the activity. Usually, this pooling step discards the temporal order of the frames, which could otherwise be used for better recognition. Towards this end, we propose a novel pooling method, generalized rank pooling (GRP), that takes as input, features from the intermediate layers of a CNN that is trained on tiny sub-sequences, and produces as output the parameters of a subspace which (i) provides a low-rank approximation to the features and (ii) preserves their temporal order. We propose to use these parameters as a compact representation for the video sequence, which is then used in a classification setup. We formulate an objective for computing this subspace as a Riemannian optimization problem on the Grassmann manifold, and propose an efficient conjugate gradient scheme for solving it. Experiments on several activity recognition datasets show that our scheme leads to state-of-the-art performance.

==> background.tex <==
\section{Background}
\label{sec:background}

\subsection{Rank Pooling}
Rank pooling~\cite{Bilen2016} is a scheme to compactly represent a sequence of video frames into a single 'image' that summarizes the pixel dynamics in the video. Typically, rank pooling solves the following objective:
\begin{equation}
\min_{z} \half\enorm{z}^2 + \sum_{i<j} \max(0, z^T x_i -z^T x_j-1)),
\end{equation}
where $x_i$ and $x_j$ are two frames from the sequence indexed by $i$ and $j$. Note that rank pooling in this framework uses a linear inner product on the original features $x$.

One shortcoming of this formulation is that there is no guarantee that the learned representation will capture other important information present in the video. For example, there could be context in the video (such as background or objects in the scene) that do not `move' and thus might not be captured in the resulting representation. In this paper, we propose a scheme to rectify this issue via learning a low-rank approximation of the input data, simultaneously conforming to their temporal order. We use this low-rank approximation as a descriptor for the data, to be used in a classifier subsequently.

